Optimizing Placement of Heap Memory Objects in Energy-Constrained Hybrid Memory Systems

Main memory (DRAM) significantly impacts the power and energy utilization of the overall server system. Non-Volatile Memory (NVM) devices, such as Phase Change Memory and Spin-Transfer Torque RAM, are suitable candidates for main memory to reduce energy consumption. But unlike DRAM, NVMs access latencies are higher than DRAM and NVM writes are more energy sensitive than DRAM write operations. Thus, Hybrid Main Memory Systems (HMMS) employing DRAM and NVM have been proposed to reduce the overall energy depletion of main memory while optimizing the performance of NVM. This paper proposes eMap, an optimal heap memory object placement planner in HMMS. eMap considers the object-level access patterns and energy consumption at the application level and provides an ideal placement strategy for each object to augment performance and energy utilization. eMap is equipped with two modules, eMPlan and eMDyn. Specifically, eMPlan is a static placement planner which provides one time placement policies for memory object to meet the energy budget while eMDyn is a runtime placement planner to consider the change in energy limiting constraint during the runtime and shuffles the memory objects by taking into account the access patterns as well as the migration cost in terms of energy and performance. The evaluation shows that our proposed solution satisfies both the energy limiting constraint and the performance. We compare our methodology with the state-of-the-art memory object classification and allocation (MOCA) framework. Our extensive evaluation shows that our proposed solution, eMPlan meets the energy constraint with 4.17 times less costly and reducing the energy consumption up to 14% with the same performance. eMDyn also satisfies the performance and energy requirement while considering the migration cost in terms of time and energy.

==> moca.tex <==
In these experiments, we modified the MOCA methodology and configure it to meet the energy constraint and then present the analysis of the cost that MOCA required to meet the energy requirements.
In Narayan et. al propsed MOCA~\cite{moca}, objects which have high LLC MPKI values are allocated to high-bandwidth and low-latency memory module, while the object which exhibits low LLC MPKI values are allocated to low-power memory based on a specific threshold.
The LLC MPKI threshold is derived from several experiments for efficient performance while maintaining energy consumption.
MOCA can also satisfy the energy limiting constraints if we set the LLC MPKI threshold effectively.
However, MOCA cannot estimate the amount of energy consumed by each object in DRAM and NVM based binary HMMS because it does not consider the details object access patterns and NVM device characteristics.
Through MOCA, the threshold to satisfy the energy constraint cannot be calculated but it must be empirically find out by performing several experiments repeatedly.
\begin{figure}[t!]
	\centering
	\includegraphics[height=0.25\textwidth, width=0.3\textwidth]{moca_energy.pdf}
	\caption{PBBS BFS Execution Time \& Energy Consumption Estimation of MOCA on Various LLC MPKI Values. (Estimated energy consumption is normalized to All-DRAM energy)}
	\label{fig_eval_moca_energy}
\end{figure}

MOCA samples the LLC MPKI and ROBH stall cycle information at a fixed interval (i.e. 1000 instructions) when the target application is executed and records the information along with the call-stack. 
After application execution is finished, MOCA maps those information to the object via allocation function call-stack, and then calculates the memory object energy consumption with per-object information. 
That is, if we assume that MOCA uses object access pattern profiling and energy models of DRAM and NVM in this research, MOCA can calculate the total energy consumption after the execution of the target application.

Figure~\ref{fig_eval_moca_energy} shows the estimated energy consumption based on various LLC MPKI values of MOCA placement in the PBBS BFS. 
%In M\_$Thr$ on the X axis, $Thr$ is the LLC MPKI value that is the threshold in placement. 
The X-asis of the figure shows the LLC MPKI threshold for the placements, M\_$Thr$. 
%As shown in Figure~\ref{fig_eval_moca_energy}, if the threshold LLC MPKI varies by same unit, change on energy consumption does not have any consistent pattern. 
As Figure~\ref{fig_eval_moca_energy} shows, if the LLC MPKI threshold varies by same unit, then the change on energy consumption does not have any consistent pattern.
Thus, to find the LLC MPKI value satisfying the energy limit constraint through MOCA, the $Thr$ should be searched by a certain unit to find a value that meets the energy constraint. 
For example, to make MOCA to meet the energy constraint that consumes less than 75\% of energy when all objects are placed in DRAM, as in Figure~\ref{fig_eval_moca_energy}, MOCA should search the correct LLC MPKI threshold by increasing current LLC MPKI value in same unit. 
If the unit is set to 0.01, MOCA must execute the target application with using the LLC MPKI value to 0.02, 0.03, 0.04, and 0.05. 
In our experimental environment, $eMap_{Static}$% module takes up to 23.635 seconds of placement computation time and object allocator overhead. 
On the other hand, MOCA should execute the application four times, which takes 78 seconds, to find the adequate LLC MPKI threshold to meet the energy constraint. 
With including real execution time that takes 20.6 seconds in M\_0.05, MOCA placement spends 4.17 times more than eMap execution time in this example.

Also, there are cases where the fluctuation of LLC MPKI threshold value, which affects energy consumption and performance, is extremely small. 
In the case of NPB CG, for example, when the LLC MPKI threshold is 0.0024, the execution takes 68.715 seconds and its energy consumption is equivalent to 91.9\% of All-DRAM placement. 
But, when the LLC MPKI threshold is lowered to 0.0023, the execution takes 42.473 seconds and consumes 95.1\% of energy of all-DRAM. 
If the energy consumption limit less than 92\% of All-DRAM is required, the effective LLC MPKI threshold can be obtained by performing LLC MPKI value search in units of 0.0001. 
When the search is performed in smaller unit, the search overhead increases accordingly.

When the energy limit constraint is satisfied in MOCA, the above processes should be repeated every time when the energy limit is changed. 
Therefore, we conclude that MOCA is not suitable for both optimizing the performance and satisfying the energy limit constraints by placing memory objects.
